The Tangent Exponential Model

The likelihood function is central to both frequentist and Bayesian formulations of parametric statistical inference, and large-sample approximations to the sampling distributions of estimators and test statistics, and to posterior densities, are widely used in practice. Improved approximations have been widely studied and can provide highly accurate inferences when samples are small or there are many nuisance parameters. This article reviews improved approximations based on the tangent exponential model developed in a series of articles by D.~A.~S.~Fraser and co-workers, attempting to explain the theoretical basis of this model and to provide a guide to the associated literature, including a partially-annotated bibliography.

==> input-files/teachingmacros.tex <==
% LaTeX macros

% Last modified: 25/12/08

%----------------------------------------------
%  Anthony Davison, Department of Mathematics,
%  EPFL, 1015 Lausanne, Switzerland
%  00 41 21 693 5502
%  Anthony.Davison@epfl.ch
%----------------------------------------------

% teaching macros

\def\redbf#1{{\color{red}\bf #1}}%
\def\red#1{{\color{red} #1}}%
\def\b#1{{\color{red}\bf #1}}%
\def\Defn{\redbf{Definition:\ }}%
\def\Thm#1{\redbf{Theorem #1:\ }}%
\def\Ex#1{\redbf{Example #1:\ }}%
\def\Note{\redbf{Note:\ }}%
\def\Exercise#1{\redbf{Exercise #1:\ }}%
\def\Ill{\redbf{Illustration:\ }}%
\def\endex{{\hfill\square\bigskip}}
\def\eme{{\`eme}}
\def\ere{{\`ere}}

\def\picbox#1#2#3{{\centerline{\psfig{figure=#1,height=#2pc,angle=#3}}}}%

\def\tt#1{{\texttt{#1}}}
\def\Der#1{\textbf{D#1}}

\def\pr{{\rm P}}

\newtheorem{defn}{Definition}
\newtheorem{alg}[defn]{Algorithm}
\newtheorem{theorem}[defn]{Theorem}
\newtheorem{lemma}[defn]{Lemma}
\newtheorem{example}[defn]{Example}
\newtheorem{cor}[defn]{Corollary}

\def\ssim{{\ {\buildrel s\over \sim}\ }}
\def\vsim{{\ {\buildrel v\over \sim}\ }}

\def\halfback{{\vspace{-0.1in}}}
\def\back{{\vspace{-0.2in}}}

\def\side{{\hspace{0.2in}}}
\def\back{{\vspace{-0.2in}}}

